Retargeting GCC: Do We Reinvent the Wheel Every Time?

Porting GCC to new architecture requires writing a Machine Description (MD) file that contains mapping from GCC's intermediate form to the target assembly code. Constructing an MD file is a difficult task because it requires the user to understand both (a) the internals of GCC, and (b) the intricacies of the target architecture. Instruction sets of different architectures exhibit significant amount of semantic similarities across a large class (for example, the instruction sets for RISC architectures) and differ only in syntax. Therefore, it is expected that MD files of machines with similar architectures should also have similarities. To confirm our hypothesis, we created "mdcompare", a tool to (a) extract RTL patterns (machine independent abstraction of RTL templates) from MD files of well known architectures and (b) compare the similarity of patterns across architectures. The results are encouraging; we found that 28% -- 70% RTL expressions are similar across pairs of MD files, the similarity percentage being on the higher side for pairs of similar architectures.

==> GCC_RTL.tex <==
\subsection{RTL Expressions}

The RTL expressions used by GCC are classified into several
classes. The classification is based on the type of their
operation and their operands. Below is a list of RTL classes
along with a brief description about each of
them\cite{gccint}.
\begin{itemize}
 \item RTX\_OBJ: An RTX code that represents an actual
   object, such as a register (reg) or a memory location
   (mem, symbol\_ref).
 \item RTX\_CONST\_OBJ: An RTX code that represents a
   constant object.
 \item RTX\_COMPARE: An RTX code for a non-symmetric
   comparison, such as geu and lt.
 \item RTX\_COMM\_COMPARE: An RTX code for a symmetric
   (commutative) comparison, such as eq, ordered, etc.
 \item RTX\_UNARY: An RTX code for a unary arithmetic
   operation, such as neg, not, abs, etc. This category also
   includes value extension (sign or zero) and conversions
   between integer and floating point.
 \item RTX\_COMM\_ARITH: An RTX code for a commutative binary
   operation, such as plus, and, ne, eq, etc.
 \item RTX\_BIN\_ARITH: An RTX code for a non-commutative
   binary operation, such as minus, div, ashiftrt, etc.
 \item RTX\_BITFIELD\_OPS: An RTX code for a bit-field
   operation. Currently only zero\_extract and sign\_extract
   are part of it.
 \item RTX\_TERNARY: An RTX code for other three input
   operations. Currently only if\_then\_els, vec\_merge,
   sign\_extract, zero\_extract, and fma are included.
 \item RTX\_INSN: An RTX code for an entire instruction.
 \item RTX\_MATCH: An RTX code for something that matches in
   insns, such as match\_dup. These only occur in machine
   descriptions.
 \item RTX\_AUTOINC: An RTX code for an auto-increment
   addressing mode, such as post\_inc.
 \item RTX\_EXTRA: All other RTX codes. This category
   includes the remaining codes used only in machine
   descriptions (define\_*, etc.). It also includes all the
   codes describing side effects (set, use, clobber, etc.)
   and the non-insns that may appear on an insn chain, such
   as note, barrier, and code\_label. subreg is also part of
   this class.
\end{itemize}


From the above list, the obvious choices for classes of RTL
expressions which will be part of the patterns are,

\begin{itemize}
 \item RTX\_COMPARE
 \item RTX\_COM\_COMPARE
 \item RTX\_UNARY
 \item RTX\_COMM\_ARITH
 \item RTX\_BITFIELDS\_OPS
 \item RTX\_TERNARY
 \item RTX\_AUTOINC
\end{itemize}
 
Apart from this, the form of an RTL expression contains a few RTL expressions from the class RTX\_EXTRA. They are called \emph{Side Effect Expressions}. They are so named, 
because they change the state of the machine. Side effect expressions include operators {\tt set}, {\tt return}, {\tt call}, {\tt clobber}, {\tt use}, {\tt parallel}, 
{\tt cond\_exec}, {\tt sequence}, {\tt asm\_input}, {\tt unspec}, {\tt unspec\_volatile}, {\tt addr\_vec} and {\tt addr\_diff\_vec}.

An \emph{internal node} of a tree is that node that has child
nodes. We have seen quite a few examples where the RTL
expressions and templates where represented as trees.  The
RTL expressions that are part of the pattern are those that
appear as internal nodes in the tree form of the RTL
expressions. The RTL expressions which are leaves in an RTL
tree form, are constants, registers or memory locations which
are chosen in a machine specific way. In summary, the RTL
expressions which are part of the pattern, tells what
operation is being done, and this has the same meaning across
machines.

So, to extract the pattern from an RTL template, we must
traverse the tree form of it and retain all nodes which form
part of the pattern and create holes in place of nodes which
are machine specific.

The list of unique patterns encountered in a MD file are
listed in a file, along with the following details.

\begin{itemize}
 \item The code iterators used in the machine. This is
   important, because the code iterators acts as aliases to
   operators and this alias is specific to a particular
   machine. So reading the patterns back won't make much
   sense without the code iterators listed.
\item The height of the pattern. The height here is height of
  the tree that represents this pattern.
\item The number of times this particular pattern is
  encountered in the files that are parsed.
\item The total number of RTL templates considered for
  parsing.
\end{itemize}




==> Makefile <==
TGT=gcc_retarget
DEPS=   gcc_retarget.bib \
	GCC_Introduction.tex \
	GCC_Related.tex \
	GCC_Methodology.tex \
	GCC_Results.tex \
	GCC_Conclusion.tex \
	fig-motivating.tex \
	fig-reuse-pattern.tex 


LATEX=pslatex
BIBTEX=bibtex
DVIPDF=dvipdf

pdf: $(TGT).pdf

$(TGT).pdf: $(TGT).tex $(DEPS)
	$(LATEX) $(TGT) && $(LATEX) $(TGT)
	$(BIBTEX) $(TGT)
	$(LATEX) $(TGT) && $(LATEX) $(TGT)
	$(DVIPDF) $(TGT).dvi

.PHONY: clean clobber fresh
clean: 
	-$(RM) -f $(TGT).dvi $(TGT).aux $(TGT).log
	-$(RM) -f $(TGT).toc $(TGT).idx $(TGT).bbl
	-$(RM) -f $(TGT).toc $(TGT).ind $(TGT).blg 
	-$(RM) -f $(TGT).ps $(TGT).ind $(TGT).pdf 
	-$(RM) -f missfont.log *~

clobber: clean
	-$(RM) -f $(TGT).ps $(TGT).pdf

fresh: clobber pdf


==> fig-reuse-pattern.tex <==
\newcommand{\Ga}{%
\scalebox{.95}{
    \psset{unit=1mm}
    \begin{pspicture}(0,0)(42,25)
      %\psframe(0,0)(42,25)
      \putnode{n0}{origin}{14}{21}{\pscirclebox{set}}
      \putnode{n1}{n0}{-10}{-9}{\psovalbox[framesep=0]{\mcspec{\$arg0}}}
      \putnode{n2}{n0}{10}{-9}{\psovalbox[framesep=0]{plus:\mcspec{\$mode}}}
      \putnode{n3}{n2}{-10}{-9}{\psovalbox[framesep=0]{\mcspec{\$arg1}}}
      \putnode{n4}{n2}{10}{-9}{\psovalbox[framesep=0]{\mcspec{\$arg2}}}
      \ncline[nodesepA=-1,nodesepB=-.5]{-}{n0}{n1}
      \ncline[nodesepA=-1]{-}{n0}{n2}
      \ncline[nodesepB=-.5]{-}{n2}{n3}
      \ncline[nodesepB=-.5]{-}{n2}{n4}
  \end{pspicture}}
  %% \begin{tabular}[b]{@{}l@{}}
  %%   [(set \mcspec{\$arg0}  (plus:\mcspec{\$mode}
  %%     \mcspec{\$arg1} \\
  %%     \rule{32.2mm}{0pt}\mcspec{\$arg2}))] \\
  %% \end{tabular}
}
\newcommand{\Gb}{%
\scalebox{.95}{
    \psset{unit=1mm}
    \begin{pspicture}(0,0)(45,35)
      %\psframe(0,0)(42,25)
      \putnode{n0}{origin}{14}{31}{\pscirclebox{set}}
      \putnode{n1}{n0}{-10}{-9}{\psovalbox[framesep=0]{\mcspec{\$arg0}}}
      \putnode{n2s}{n0}{17}{-9}{\psovalbox[framesep=0]{sign\_extend:\mcspec{\$mode}}}
      \putnode{n2}{n2s}{0}{-9}{\psovalbox[framesep=0]{plus:\mcspec{\$mode}}}
      \putnode{n3}{n2}{-10}{-9}{\psovalbox[framesep=0]{\mcspec{\$arg1}}}
      \putnode{n4}{n2}{10}{-9}{\psovalbox[framesep=0]{\mcspec{\$arg2}}}
      \ncline[nodesepA=-1,nodesepB=-.5]{-}{n0}{n1}
      \ncline[nodesepA=-.5]{-}{n0}{n2s}
      \ncline[nodesepB=-.5]{-}{n2s}{n2}
      \ncline[nodesepB=-.5]{-}{n2}{n3}
      \ncline[nodesepB=-.5]{-}{n2}{n4}
  \end{pspicture}}
  %% \begin{tabular}[b]{@{}l@{}}
  %%   [(set \mcspec{\$arg0} 
  %%     (sign\_extend:\mcspec{\$mode}  \\
  %%     \rule{20.5mm}{0pt}(plus:\mcspec{\$mode} \mcspec{\$arg1} \\
  %%     \rule{37.6mm}{0pt}\mcspec{\$arg2})))] \\
  %% \end{tabular}
}
\newcommand{\Gc}{
\scalebox{.95}{
    \psset{unit=1mm}
    \begin{pspicture}(0,0)(45,44)
      %\psframe(0,0)(42,25)
      \putnode{n0}{origin}{14}{40}{\pscirclebox{set}}
      \putnode{n1}{n0}{-10}{-9}{\psovalbox[framesep=0]{\mcspec{\$arg0}}}
      \putnode{n2s}{n0}{17}{-9}{\psovalbox[framesep=0]{zero\_extend:\mcspec{\$mode}}}
      \putnode{n2s1}{n2s}{0}{-9}{\psovalbox[framesep=0]{subreg:\mcspec{\$mode}}}
      \putnode{n2}{n2s1}{-11}{-9}{\psovalbox[framesep=0]{plus:\mcspec{\$mode}}}
      \putnode{s2}{n2s1}{11}{-9}{\psovalbox[framesep=0]{\mcspec{\$offset}}}
      \putnode{n3}{n2}{-10}{-9}{\psovalbox[framesep=0]{\mcspec{\$arg1}}}
      \putnode{n4}{n2}{10}{-9}{\psovalbox[framesep=0]{\mcspec{\$arg2}}}
      \ncline[nodesepA=-1,nodesepB=-.5]{-}{n0}{n1}
      \ncline[nodesepA=-.5]{-}{n0}{n2s}
      \ncline[nodesepB=-.5]{-}{n2s}{n2s1}
      \ncline[nodesepB=-.1]{-}{n2s1}{n2}
      \ncline[nodesepB=-.1]{-}{n2s1}{s2}
      \ncline[nodesepB=-.5]{-}{n2}{n3}
      \ncline[nodesepB=-.5]{-}{n2}{n4}
  \end{pspicture}}
%\includegraphics[scale = 0.35]{G2.epsi}
}
\newcommand{\Gd}{
\scalebox{.95}{
    \psset{unit=1mm}
    \begin{pspicture}(0,0)(45,44)
      %\psframe(0,0)(42,25)
      \putnode{n0}{origin}{14}{40}{\pscirclebox{set}}
      \putnode{n1}{n0}{-10}{-9}{\psovalbox[framesep=0]{\mcspec{\$arg0}}}
      \putnode{n2s}{n0}{17}{-9}{\psovalbox[framesep=0]{zero\_extend:\mcspec{\$mode}}}
      \putnode{n2s1}{n2s}{0}{-9}{\psovalbox[framesep=0]{truncate:\mcspec{\$mode}}}
      \putnode{n2}{n2s1}{0}{-9}{\psovalbox[framesep=0]{plus:\mcspec{\$mode}}}
      \putnode{n3}{n2}{-10}{-9}{\psovalbox[framesep=0]{\mcspec{\$arg1}}}
      \putnode{n4}{n2}{10}{-9}{\psovalbox[framesep=0]{\mcspec{\$arg2}}}
      \ncline[nodesepA=-1,nodesepB=-.5]{-}{n0}{n1}
      \ncline[nodesepA=-.5]{-}{n0}{n2s}
      \ncline[nodesepB=-.5]{-}{n2s}{n2s1}
      \ncline[nodesepB=-.1]{-}{n2s1}{n2}
      \ncline[nodesepB=-.5]{-}{n2}{n3}
      \ncline[nodesepB=-.5]{-}{n2}{n4}
  \end{pspicture}}
%\includegraphics[scale = 0.35]{G3.epsi}}
}
\begin{table}[t]
  \centering
  \caption{Summary of Patterns for variations in {\em add}
    instruction from MIPS MD file. Numbers in parentheses
    denote the occurrences of patterns.
  \label{tab:addsummary}}
  \scalebox{.79}{
    \begin{tabular}{@{}|@{}r@{}|@{}r@{}|@{}}
      \hline
      {\Ga} (17) & {\Gb} (2)\\      \hline
      {\Gc}  (2) & {\Gd} (1)\\      \hline
  \end{tabular}}
\end{table}

